Text2Chart31: Instruction Tuning for Chart Generation with Automatic Feedback

Large language models (LLMs) have demonstrated strong capabilities across various language tasks, notably through instruction-tuning methods. However, LLMs face challenges in visualizing complex, real-world data through charts and plots. Firstly, existing datasets rarely cover a full range of chart types, such as 3D, volumetric, and gridded charts. Secondly, supervised fine-tuning methods do not fully leverage the intricate relationships within rich datasets, including text, code, and figures. To address these challenges, we propose a hierarchical pipeline and a new dataset for chart generation. Our dataset, Text2Chart31, includes 31 unique plot types referring to the Matplotlib library, with 11.1K tuples of descriptions, code, data tables, and plots. Moreover, we introduce a reinforcement learning-based instruction tuning technique for chart generation tasks without requiring human feedback. Our experiments show that this approach significantly enhances the model performance, enabling smaller models to outperform larger open-source models and be comparable to state-of-the-art proprietary models in data visualization tasks. We make the code and dataset available at https://github.com/fatemehpesaran310/Text2Chart31.

==> tables/table1.tex <==

\begin{center}
\begin{table*}[t]
\caption{Comparison with other datasets: PlotQA \citep{methani2020plotqa}, ChartQA \cite{masry2022chartqa}, FigureQA \cite{kahou2018figureqa},
Unichart \cite{masry2023unichart}, Autochart \cite{zhu2021autochart}, Chart-to-Text \cite{kantharaj2022charttotext}, and ChartLlama \cite{han2023chartllama}. The Text-to-Chart task has been split into three sub-tasks: \textbf{(1) \textit{Description-to-Chart}}: Generate a chart from a natural language description using data either within the description only or from a linked CSV file. \textbf{(2) \textit{Raw Data-to-Chart:}} Analyze raw data from a CSV file and generate the most suitable chart based on the data analysis. \textbf{(3) \textit{Code-to-Description}}: Given the visualization code of the chart, generate the description of the chart. *ChartLlama consists of both Chart-To-Text and Text-to-Chart, and we present the latter part for better comparison with our dataset.
$^\dagger$\textit{Distinct-n:} We calculate average distinct-n grams for $n$ from 1 to 5\citep{li2016diversitypromoting}.
$^\ddagger$ To measure the dataset balance score, we use Shannon Diversity Index \citep{friedman2023vendi}. \textcolor{red}{Gunhee Kim: It seems you are ignoring other dataset's strong points. Change the table in a fair way. Creating the table to your own favour can be viewed as manipulation!. And try to emphasize on why generating these new types of plots are important for LLMs.}}
\label{tab:comparison}
\centering
\begin{adjustbox}{max width=2.0\columnwidth}
\begin{tabular}{l  c c c c c  c  c  c c}
\toprule
& \multicolumn{2}{c}{\small{\textbf{\# Data }}} 
& \multicolumn{4}{c}{\small{\textbf{\# Plot Type }}} 
& \multicolumn{2}{c}{\small{\textbf{Quality Analysis}}} \\
\cmidrule(lr){1-1}
\cmidrule(lr){2-3}
\cmidrule(lr){4-7} 
\cmidrule(lr){8-9}

%%%%%%%%%%%%%%%%%%%%%
\small{{\textbf{Dataset}}}& \shortstack{\scriptsize{\textbf{Description}} \\ \scriptsize{\textbf{to Chart}}} & \shortstack{\scriptsize{\textbf{Raw Data}} \\ \scriptsize{\textbf{to Chart}} } & 
\shortstack{\scriptsize{\textbf{Pairwise\&}} \\ \scriptsize{\textbf{Statistical}} \\ \scriptsize{\textbf{Dist. Data}}} & 
\shortstack{\scriptsize{\textbf{Gridded\&}} \\ \scriptsize{\textbf{Irregularly}} \\ \scriptsize{\textbf{ Gridded Data}}} &
\shortstack{\scriptsize{\textbf{3D\&}} \\ \scriptsize{\textbf{Volumetric}}
\\ \scriptsize{\textbf{Data}}}
&\scriptsize{\textbf{Total}}& \shortstack{ \scriptsize{\textbf{Dataset}} \\ \scriptsize{\textbf{Balance}} \\ \scriptsize{\textbf{Score}$^\ddagger$} } &  \shortstack{\scriptsize{\textbf{Content}}\\ \scriptsize{\textbf{Diversity}} \\ \scriptsize{\textbf{(\textit{Distinct-n}$^\dagger$)}}}\\ 
%%%%%%%%%%%%%%%%%%%%%

% \cmidrule(lr){1-1}
% \cmidrule(lr){2-3}
% \cmidrule(lr){4-7} 
% \cmidrule(lr){8-9}

\cmidrule(lr){1-1}
\cmidrule(lr){2-3}
\cmidrule(lr){4-7} 
\cmidrule(lr){8-9}
\multicolumn{3}{l}{\small{\textit{\textbf{Chart-to-Text Domain}}}} &  &  &  &  &  & \\

\small{PlotQA} & \small{-} & \small{-} & \small{3} & \small{\xmark}& \small{\xmark} &\small{3} & \small{0.786} &  \small{0.038} \\

\small{ChartQA} & \small{-} & \small{-} & \small{3} & \small{\xmark}& \small{\xmark} &\small{2} & \small{0.422} &  \small{-} \\

\small{FigureQA} & \small{-}& \small{-} & \small{4} & \small{\xmark} & \small{\xmark} & \small{4} & \small{0.960} &  \small{-} \\

\small{Unichart} & \small{-} & \small{-} & \small{3} & \small{\xmark} &\small{\xmark} & \small{3} & \small{-} &  \small{0.157}\\

\small{AutoChart} & \small{-} & \small{-} & \small{3} & \small{\xmark} &\small{\xmark} & \small{3} & \small{0.978} & \small{0.027}\\


\small{Chart-to-Text} & \small{-} & \small{-} &  \small{5} & \small{1} & \small{\xmark} & \small{6} & \small{0.326} & \small{0.510}\\
\cmidrule(lr){1-1}
\cmidrule(lr){2-3}
\cmidrule(lr){4-7} 
\cmidrule(lr){8-9}
\multicolumn{3}{l}{\small{\textit{\textbf{Text-to-Chart Domain}}}} &  &  &  &  &  & \\
\small{ChartLlama*} &  \small{7.84k} & \small{\xmark}  & \small{8}  & \small{2} & \small{\xmark} & \small{10} & \small{0.738} & \small{-}\\
\cmidrule(lr){1-1}
\cmidrule(lr){2-3}
\cmidrule(lr){4-7} 
\cmidrule(lr){8-9}

\small{\textbf{T4C31 (Ours)}} & \small{\textbf{10.5k}} & \small{\textbf{7.6k}}  & \small{\textbf{16}}  & \small{\textbf{10}} & \small{\textbf{5}} & \small{\textbf{31}} & \small{\textbf{0.981}} & \small{\textbf{0.674}} \\
\bottomrule
\end{tabular}
\end{adjustbox}

\end{table*}
\end{center}


